Symmetry-Informed Governing Equation Discovery

Despite the advancements in learning governing differential equations from observations of dynamical systems, data-driven methods are often unaware of fundamental physical laws, such as frame invariance. As a result, these algorithms may search an unnecessarily large space and discover less accurate or overly complex equations. In this paper, we propose to leverage symmetry in automated equation discovery to compress the equation search space and improve the accuracy and simplicity of the learned equations. Specifically, we derive equivariance constraints from the time-independent symmetries of ODEs. Depending on the types of symmetries, we develop a pipeline for incorporating symmetry constraints into various equation discovery algorithms, including sparse regression and genetic programming. In experiments across diverse dynamical systems, our approach demonstrates better robustness against noise and recovers governing equations with significantly higher probability than baselines without symmetry. Our codebase is available at https://github.com/Rose-STL-Lab/symmetry-ode-discovery.

==> sec/ete.tex <==
\section{End-to-End Pipeline}
In the previous section, we demonstrated the efficacy of ESINDy in discovering equivariant equations from dynamical systems. However, these experiments were based on the assumption that we had prior knowledge of the system's inherent symmetries, which allowed us to input the corresponding Lie algebra basis $L_i$ into our model. Nonetheless, it is challenging in real-world applications. More often than not, we do not know the underlying symmetries of an unknown dynamical system in advance, which hinders the practical application of ESINDy model.

\subsection{Combination of LieGAN and ESINDy}
LieGAN \cite{yang23} is designed to autonomously discover symmetries within a dataset using a paradigm similar to generative adversarial training, and yield the corresponding Lie algebra basis, which is exactly what ESINDy requires as input. Therefore, we propose a combination of LieGAN and ESINDy to form an end-to-end pipeline. This integration automates the entire process, from symmetry discovery within the dataset to the derivation of corresponding equivariant governing equations.

\subsection{Experiments for End-to-end Pipeline}
\paragraph{Lotka-Volterra System.}
The dynamic interactions between predators and prey can be described by a set of nonlinear ODEs, known as the Lotka-Volterra equations. We focus on their standard form:

\begin{equation}
\label{eq_lv}
\left\{
\begin{aligned}
    \dot p &= a - b e ^ q  \\
    \dot q &= c e ^ p - d
\end{aligned}
\right.
\end{equation}
    


In these equations, $p$ and $q$ correspond to the logarithm of population densities of prey and predator, respectively. The parameters $a, b, c, d$ are indicators of population growth and mortality rates. For our experiment, we set $a$ to $2/3$, $b$ to $4/3$, and both $c$ and $d$ to $1$. We generate $N=200$ trajectories spanning $T=10^4$ timesteps with a timestep interval $\Delta t=0.002$.


